Instance Selection for Dynamic Algorithm Configuration with Reinforcement Learning: Improving Generalization

Dynamic Algorithm Configuration (DAC) addresses the challenge of dynamically setting hyperparameters of an algorithm for a diverse set of instances rather than focusing solely on individual tasks. Agents trained with Deep Reinforcement Learning (RL) offer a pathway to solve such settings. However, the limited generalization performance of these agents has significantly hindered the application in DAC. Our hypothesis is that a potential bias in the training instances limits generalization capabilities. We take a step towards mitigating this by selecting a representative subset of training instances to overcome overrepresentation and then retraining the agent on this subset to improve its generalization performance. For constructing the meta-features for the subset selection, we particularly account for the dynamic nature of the RL agent by computing time series features on trajectories of actions and rewards generated by the agent's interaction with the environment. Through empirical evaluations on the Sigmoid and CMA-ES benchmarks from the standard benchmark library for DAC, called DACBench, we discuss the potentials of our selection technique compared to training on the entire instance set. Our results highlight the efficacy of instance selection in refining DAC policies for diverse instance spaces.

==> nomclat.tex <==
% Everything supposed to be used in equation mode?
% use in preamble: \input{macros_DAC.tex}

% Necessary packages for definitions
\usepackage{amsmath}
\usepackage{mathtools}  % for :=
\usepackage{amsfonts} 

\newcommand{\code}[1]{\small{\texttt{#1}}} 

%beginmacros

%--------- General Math Notation
\DeclareMathOperator*{\E}{\mathbb{E}}           % Expectation as a math operator
\DeclareMathOperator*{\expectation}{\mathbb{E}} % Expectation as a math operator
\renewcommand{\vec}[1]{\mathbf{#1}}             % Bold emphasis for vectors
\DeclareMathOperator*{\argmin}{arg\,min}        % Argmin
\DeclareMathOperator*{\argmax}{arg\,max}        % Argmax
\newcommand{\natnums}{{\mathbb{N}}}              % Notation for set of natural numbers
\newcommand{\realnums}{{\mathbb R}}             % Notation for set of real numbers
\newcommand{\extset}[2]{\{#1 \; | \; #2\}}      % Set of a given b. Renders {{a | b}}.    
\newcommand{\ddfrac}[2]{\frac{\displaystyle #1}{\displaystyle #2}}    % Double Display Fraction, forces large displays for everything in numerator and denominator

\newcommand{\diff}{\mathop{}\!\mathrm{d}}       % ???????
\newcommand{\transpose}[0]{{\textrm{\tiny{\sf{T}}}}} % Transpose T. Usage: $A^\transpose$
\newcommand{\norm}{{\mathcal{N}}}               % Normal distribution
\newcommand{\normaldist}{{\mathcal{N}}}         % Normal distribution
\newcommand{\iter}[2][\bocount]{{#2}^{(#1)}}    % Iteration specific instance of variable/function/anything

%-- Stochastic
\newcommand{\pdf}{\phi}                         % Standard Normal PDF
\newcommand{\cdf}{\Phi}                         % Standard Normal CDF
\newcommand{\mean}{\mu}                         % Mean
\newcommand{\stddev}{\sigma}                    % Standard Deviation
\newcommand{\variance}{\sigma^2}                % Variance
\newcommand{\noise}{\nu}                        % Noise
\newcommand{\given}[1][]{\:#1\vert\:}           % Conditional Probability "Given That" Relation, source: https://tex.stackexchange.com/a/141685/205886
\newcommand{\prob}[0]{p}                        % Probability p
\newcommand{\Prob}[0]{P}                        % Probability distribution P


%------- Notation for Configuration(s)

\newcommand{\confspace}[0]{\pmb{\Lambda}}       % Configuration space of parameters
\newcommand{\conf}[0]{\pmb{\lambda}}            % Configuration of parameters
%\newcommand{\bx}[0]{\conf}                     % Configuration of parameters
\newcommand{\hyperparam}{\lambda}               % Single hyperparameter of configuration
\newcommand{\hyperparami}[1][i]{{\hyperparam}_{#1}}   % Single hyperparameter within a hyperparameter configuration
\newcommand{\confinc}[0]{\pmb{\hat{\lambda}}}   % Incumbent configuration
%\newcommand{\confI}[1]{{\conf}^{(#1)}}      % Configuration corresponding to a given iteration -- better use \iter!
\newcommand{\confdef}[0]{{\conf}_{\text{def}}}  % Default configuration
\newcommand{\incumbent}[1][\bocount]{\iter[#1]{\confinc}}   % Incumbent configuration
\newcommand{\confincfin}{\incumbent[\bobudget]} % Final incumbent configuration (at end of run)
\newcommand{\confopt}[0]{{\conf}^*}             % Optimal configuration


%------- Notation for Cost, Risk, Loss, Performance Metric or Objective Functions

\newcommand{\loss}[0]{\mathcal{L}}              % Loss
\newcommand{\risk}{\mathcal{R}}                 % Risk
\newcommand{\riskemp}{\mathcal{R}_{\text{emp}}} % Empirical risk
\newcommand{\cost}[0]{c}                        % Cost
\newcommand{\costi}[1]{c^{(#1)}}                % Cost of instance/identifier
\newcommand{\objF}{F}                           % Family of objective functions
\newcommand{\func}[0]{f}                        % Function
\newcommand{\perfdomain}[0]{\mathbb{R}}         % Performance domain


%------- Notation for Algorithms
\newcommand{\algo}[0]{A}                        % One algorithm
\newcommand{\algos}[0]{\mathbf{A}}              % Set of algorithms    


\newcommand{\feat}[0]{\x_{\text{meta}}}                 % Meta features
\newcommand{\feats}[0]{\mathcal{X}_{\text{meta}}}       % Set of meta features


%------- Notation for Machine Learning
\newcommand{\dset}[0]{\mathcal{D}}                          % Dataset (instance)
\newcommand{\dsetmeta}[0]{\dset_{\text{meta}}}              % Dataset: meta
\newcommand{\dsettrain}[0]{\dset_{\text{train}}}            % Dataset: train
\newcommand{\dsetval}[0]{\dset_{\text{val}}}                % Dataset: val
\newcommand{\dsettest}[0]{\dset_{\text{test}}}              % Dataset: test
\newcommand{\x}[0]{\mathbf{x}}                              % Input vector x
\newcommand{\y}[0]{y}                                       % Output y
\newcommand{\xI}[1]{\mathbf{x}^{(#1)}}                      % i-th component of input
\newcommand{\yI}[1]{y^{(#1)}}                               % i-th component of output
\newcommand{\fx}{f(\mathbf{x})}                             % f(x), continuous prediction function
\newcommand{\Hspace}{\mathcal{H}}                           % hypothesis space where f is from
\newcommand{\fh}{\hat{f}}                                   % f hat, estimated prediction function


%------- Notation for Deep Learning
\newcommand{\weights}[0]{\mathbf{\theta}}                   % Weights of neural network
\newcommand{\metaweights}[0]{\phi}                          % Weights of a meta-network


%------- Notation for AutoML
\newcommand{\portfolio}[0]{\mathbf{P}}                      % Portfolio
\newcommand{\schedule}[0]{\mathcal{S}}                      % Schedule
\newcommand{\hist}[0]{\dset_{\text{hist}}}                  % History


%------- Notation for Bayesian Optimization
%-- Components
\newcommand{\GP}{\mathcal{G}}                   % Gaussian Process
\newcommand{\kernel}{\kappa}                    % Kernel
\newcommand{\acq}{u}                            % Acquisition Function
\newcommand{\constraintg}{g}                    % Constraint function
\newcommand{\surro}[0]{\hat{\cost}}             % Surrogate model

%-- Loop
\newcommand{\bocount}{t}                        % BO loop counter
\newcommand{\bobudget}{T}                       % BO loop counter max, the counter runs from 1 to this value
\newcommand{\obs}[1][\conf]{\cost({#1})}        % BO loop observation
\newcommand{\obsspace}{\mathcal{Y}}             % BO loop observation space
\newcommand{\bonextobs}{\obs[\iter{\conf}]}     % BO loop next observation
\newcommand{\bonextsample}{\iter{\conf}}        % BO loop next selected sample

%-- Dataset
\newcommand{\dsetHPOdef}{{\langle \bonextsample,\,\bonextobs \rangle}_{\bocount=1}^{\bobudget}}     % Observed cost for selected configurations during BO run


%------- Notation for Reinforcement Learning
%-- Markov Decision Process with Components
\newcommand{\MDP}[0]{M}                       % MDP (Markov Decision Process)
\newcommand{\statespace}[0]{\mathcal{S}}                % State space
\newcommand{\state}[0]{s}                               % State
\newcommand{\statet}[1][t]{\state_{#1}}                 % State at time t
\newcommand{\actionspace}[0]{\mathcal{A}}               % Action space
\newcommand{\actionrl}[0]{a}                            % Action
\newcommand{\transdomain}[0]{\mathcal{T}}               % Transition domain (probability distribution of algorithm state transitions)
\newcommand{\trans}[0]{t}                               % Transition
\newcommand{\rewards}[0]{\mathcal{R}}                   % Reward function
\newcommand{\reward}[0]{r}                              % Reward

\newcommand{\policies}[0]{\mathbf{\Pi}}                 % Policies
\newcommand{\policy}[0]{\pi}                            % Policy
\newcommand{\policyopt}[0]{{\policy}^*}                 % Optimal policy

\newcommand{\discount}[0]{\gamma}                       % Discount rate
\newcommand{\valueS}[0]{\mathcal{V}}                    % State value function
\newcommand{\valueSip}[1][\inst]{\valueS^{\policy}_{#1}} % State value function under policy pi and instance i
\newcommand{\Qfunc}[0]{\mathcal{Q}}                     % State action value function (Q)
\newcommand{\Qfuncip}[1][\inst]{\Qfunc^{\policy}_{#1}}  % State action value function (Q) under policy pi and instance i

\newcommand{\egreedy}[0]{$\epsilon$-greedy}             % $\egreedy$ 

\newcommand{\trajectory}{\tau}                          % Trajectory
\newcommand{\episode}[0]{\mathcal{E}}                  % Episode
\newcommand{\expreturn}[0]{G}                           % Expected return
\newcommand{\cutoff}[0]{\kappa}                         % Cutoff kappa


%-- Dynamic Algorithm Configuration (DAC)
\newcommand{\inst}[0]{i}                    % One instance
\newcommand{\insts}[0]{\mathcal{I}}         % Set of instances
\newcommand{\insti}[1]{i^{(#1)}}            % Numbered instance. Usage: $\insti{3}$ for 3rd instance.

\newcommand{\cMDP}[0]{\mathcal{M}}                      % cMDP (contextual MDP)
\newcommand{\cMDPdef}[0]{\cMDP \coloneqq \{\MDPi\}_{\inst \sim \insts}} % cMDP: Definition as set of MDPs per instance
\newcommand{\MDPi}[0]{\MDP_\inst}                       % MDP of one instance
\newcommand{\MDPidef}[0]{\MDPi \coloneqq (\statespace, \actionspace, \transdomaini, \rewardsi)}  % MDP: Definition as tuple for one instance

\newcommand{\transdomaini}[0]{\transdomain_\inst}       % Transitions (instance-specific)
\newcommand{\rewardsi}[0]{\rewards_\inst}               % Rewards (instance-specific)    
\newcommand{\curric}[0]{\mathbf{d}}                     % Curriculum
\newcommand{\contexti}[1][i]{c_{#1}}                    % Context of instance i

\newcommand{\configspaceDAC}[0]{\Theta}                 % Configuration space
\newcommand{\configDAC}[0]{\theta}                      % Configuration
\newcommand{\hyperparamset}{H}                          % Hyperparameter set
\newcommand{\hyperparamname}[0]{h}                      % Name of hyper-/configuration parameter

%endmacros


% Regret
% Return

==> performance_table.tex <==

\begin{table*}[h!]
    \caption{Performance on the Test Set. We show (lower CI, metric score, upper CI).}
    \centering
    \small{
    \resizebox{\linewidth}{!}{%
\begin{tabular}{lllllll}
\toprule
Benchmark & \multicolumn{3}{r}{Sigmoid} & \multicolumn{3}{r}{CMA-ES} \\
Metric & Median & IQM & Mean & Median & IQM & Mean \\
Origin &  &  &  &  &  &  \\
\midrule
ISA & 0.465, \textbf{0.471}, 0.474 & 0.470, \textbf{0.472}, 0.474 & 0.475, \textbf{0.477}, 0.479 & 0.720, \textbf{0.730}, 0.781 & 0.714, \textbf{0.737}, 0.757 & 0.674, \textbf{0.688}, 0.702 \\
full & 0.438, \textbf{0.441}, 0.446 & 0.441, \textbf{0.443}, 0.446 & 0.445, \textbf{0.447}, 0.448 & 0.713, \textbf{0.739}, 0.766 & 0.697, \textbf{0.716}, 0.736 & 0.667, \textbf{0.679}, 0.692 \\
random & 0.437, \textbf{0.443}, 0.445 & 0.439, \textbf{0.441}, 0.443 & 0.443, \textbf{0.445}, 0.447 & 0.692, \textbf{0.715}, 0.734 & 0.671, \textbf{0.686}, 0.700 & 0.642, \textbf{0.651}, 0.660 \\
selector & 0.438, \textbf{0.443}, 0.446 & 0.440, \textbf{0.443}, 0.446 & 0.443, \textbf{0.446}, 0.448 & 0.750, \textbf{0.771}, 0.794 & 0.744, \textbf{0.761}, 0.779 & 0.716, \textbf{0.731}, 0.746 \\
\bottomrule
\end{tabular}
}
}
    \label{tab:performance}
\end{table*}

==> reviews.tex <==
Decision: Accept as a Poster
Submission: Instance Selection for Dynamic Algorithm Configuration with Reinforcement Learning: Improving Generalization
Contributors: Benjamins, Cenikj, Eftimov, Lindauer, Mohan, Nikolikj

Key for the below column headings show
Summary of Reviews of pap418s2	
Reviewer	rel 	sig 	orig 	ach 	writ 	rep 	tech 	rec 	conf
Reviewer 1	4	4	3	4	4	3	3	3-definitely accept as poster (3)	4
Reviewer 2	4	3	3	3	3	3	2	1-definitely reject outright (1)	4
Reviewer 3	5	4	3	3	4	4	3	3-definitely accept as poster (3)	4
Reviewer 4	5	4	4	5	5	5	4	5-definitely accept as full paper (5)	3
Averages:	4.5	3.8	3.2	3.8	4.0	3.8	3.0	3.0	3.8

Sections Below

    Full Reviews · jump down
    Committee Discussion with Authors · jump down
    Committee Comments · jump down


 Full Reviews
Reviewer 1	top

Comments for Authors

    monospace
    markdown
    The paper is about selecting a set of instances that will help the generalisation of Reinforcement Learning (RL) for Dynamic Algorithm Configuration.
    The goal is to select a subset of representative instances such that RL algorithms avoid overfitting.
    The authors use two benchmarks from the DAC library to test their method and show that selecting representative sets of instances is beneficial to the performance of the hyperparameter tuning.

    Overall the paper is well written and easy to follow.
    Authors will provide code and data upon acceptance but since I cannot check it and because the pipeline is too complex to re-implement it for the review, I cannot give the highest grades for the replicability.

    I have a few comments/questions on the content:

        Authors chose to perform instance selection to achieve their goal of improving the generalisation of RL for DAC. Nevertheless, I think the related work should contain a section about instance generation as it can be used for the same purpose, i.e., generate discriminative and representative instances to help RL generalise.
        Why the choice of catch22 over other methods ? Could other methods be used ?
        Figure 3 is not easy to read.
        Why use 10 functions out of the 24 from BBOB ? Is it because only 10 are available in DAC or is it a choice ? I guess from l529 that five instances are used but it is not clearly stated.
        Why are the number of environment steps are different and why this choice of numbers ? Why for CMA-ES the episode lengths are variables ?
        From the presented results, it seems that more than one run is performed but it is not clear if the pipeline is repeated multiple times (or part of the pipeline as SELECTOR is run 5 times) or if a cross-validation is performed.
        Table 2: title and labels are not clear. What is it the performance of ? What is the performance measure ? What is IQM (used but not defined in the text) ? What is CI, confidence interval maybe ?
        For CMA-ES, is a fixed-budget or fixed-target performed ? What is the performance metric ?
        L678: “Interestingly, the performance of the ISA for CMA-ES is worse than the performance of SELECTOR”, where is this seen and why (i.e., lower median, statistical test) ?
        L743: selecting one instance only by function makes sense from the algorithm point of view as transformations of the fitness function should not impact the algorithm performance.


Scored Review Questions

	rel 	sig 	orig 	ach 	writ 	rep 	tech 	rec 	conf
pap418s2	4	4	3	4	4	3	3	3-definitely accept as poster (3)	4

Reviewer 2	top

Comments for Authors

    monospace
    This paper still needs a lot of work before making a useful contribution.
    My main concern is that the conclusions are not supported by the evidence. Particularly, the statement in the conclusion "On both benchmarks, Sigmoid and CMA-ES, training on subselected instances from SELECTOR generalizes better to the test instance set than training on the full instance set". Firstly, this is incorrect, since the evidence on Sigmoid is that there is no difference in performance (0.443 versus 0.441 for Median metric; 0.443 versus 0.433 for IQR metric, 0.446 versus 0.447 for Mean metric) - one the same, one slightly worse, one slightly better, but none of this is likely to be statistically significant (which wasn't tested). No explanation is given for my the method might not perform well on Sigmoid (in fact, it is suggested that it does). On CMA-ES the results are more convincing of the merits of selecting a subset of instances, but the chosen test functions from BBOB are all easy (separable, low conditioning), and I am not sure why all 12 BBOB functions were not chosen? It looks like perhaps the method only works well for easy functions, which limits its utility. The chosen test instances in Fig 11 were very difficult to understand (what is count referring to?), and the claim that these represent a diverse set is not supported adequately.
    Overall, the paper could be improved in how it explained the methodology, perhaps with an example showing the 2x24 inputs (columns) with instances (rows) as input to SELECTOR, and then how the MIS problem is solved to arrive at the chosen rows. The diversity of those instances needs to be better illustrated, and the dependence of the generalization performance on different random test sets (via cross validation) needs to be shown.
    The review of existing methods for instance selection that consider algorithm performance (in addition to instance features) was not comprehensive enough. I appreciate that the paper has extended the SELECTOR methodology (that uses no algorithm performance information) to use RL experience to support instance selection informed by knowledge of how parameters affect algorithm performance (recasting the DAC problem to one of RL). The idea is fine, but the paper doesn't provide enough rigorous investigation of the performance in practice of the idea.
    Fig 4 shows the test functions are very similar to the training functions, and there seems to be no concept of cross-validation used to support the results.
    The final sentences are very grand, and not appropriate for the significance of this paper's contribution.


Scored Review Questions

	rel 	sig 	orig 	ach 	writ 	rep 	tech 	rec 	conf
pap418s2	4	3	3	3	3	3	2	1-definitely reject outright (1)	4

Reviewer 3	top

Comments for Authors

    monospace
    markdown
    The paper addresses an important question in developing effective dynamic algorithm configuration (DAC) methods: how to select instances during the training such that the generalisation ability of the trained reinforcement learning (RL) agent is maximised. The authors propose using SELECTOR (Cenikj et al 2022), a method for selecting a representative subset of instances via their similarity in instance features. The features are obtained via: (i) training an RL agent on the whole training set once, (ii) evaluating the trained agent on the training instances and recording the trajectories of actions and rewards; and (iii) using those trajectories as raw instance features or extracting time series features and using them as instance features. The agent is then trained once more time using the subset of instances selected by SELECTOR to improve its performance.

    The topic the paper is addressing is important and the idea is interesting. However, there are a number of questionable points that I’d like to raise regarding the current experiment setup and the analysis.

    First, there is a potential issue with the current setting of the comparison. More concretely, the results in Figures 5 and 6 are obtained from selecting the best selector-agent among multiple ones (derived from training an agent per combination of SELECTOR’s hyper-parameter), which may raise the question of whether the comparison is fair and if the performance improvement really comes from the instance selection part. If we repeat the training of the other two agents (full-agent and random-agent) multiple times and choose the best one among them, would we be able to achieve similar performance to the tuned selector-agent? Also did you choose the best selector-agent based on its performance on the test set or the training set? If the test performance is used, it makes the comparison even more questionable.

    Second, there exists other work in the literature for selecting instances during RL training. A very relevant piece of work is:

    Eimer, T., Biedenkapp, A., Hutter, F. and Lindauer, M., 2021. Self-paced context evaluation for contextual reinforcement learning. ICML

    The instance selection method proposed in that work is directly comparable to the one proposed in this paper, but it is not mentioned or considered in the current text and analysis.

    Third, on the sigmoid benchmark, the paper claims that the selector-agent generalises better than the other two (full-agent and random-agent), but the detailed numbers and plots do not seem to support the claim (The difference in performance on the CMA-ES benchmark is clear though, and it’s interesting to see that the selector-agent performs better than the ISA-agent on the test set).

    Fourth, regarding the analysis, the authors mention that fANOVA was used for analysing the importance of hyper-parameters and refer to Hutter et al (2014) for the method. But I don’t see why that method is used here. In Hutter et al, fANOVA conducted a surrogate model to predict the performance of any algorithm configuration and used that model for computing hyper-parameter importance. However, in this setting, we have the full-factorial data (of all combinations of hyper-parameters), so there is no need for building a surrogate model on top of that. Moreover, is the importance of each hyper-parameter reported in the paper based on the marginal contributions of those hyper-parameters given by fANOVA analysis, and if it is, can we see the numbers? Finally, some hyper-parameters may deem unimportant when being considered in isolation, but they may have strong interactions with other hyper-parameters. fANOVA can also give us information about such interactions, but they are not considered in the current analysis.

    Some other minor points that could be improved or clarified further:

        How is the second RL training done (i.e., the RL training on the selected subset of instances)? Did you start PPO from scratch but seeding the best trained policy from the first training, or did you just continue the first PPO training but now with the new set of instances?

        Table 2: “Sigmoid” and “CMA-ES” could be centre-aligned for better readability.

        Typo on page 7: “We observe agin” -> again


Scored Review Questions

	rel 	sig 	orig 	ach 	writ 	rep 	tech 	rec 	conf
pap418s2	5	4	3	3	4	4	3	3-definitely accept as poster (3)	4

Reviewer 4	top

Comments for Authors

    monospace
    An approach to select instances is proposed that allows for better generalization of reinforcement learning agents, which are used to control hyperparameters of optimization algorithms. The proposed approach is well justified by the related work and shows convincing empirical results, especially for controlling step size in CMA-ES. In the latter case the proposed approach of learning on selected instances clearly outperforms learning on the full set of instances, as well as on a randomly selected subset and even the baseline method, which was meant to be the most efficient one. However, for the Sigmoid experiment, some comments on statistical significance are needed, as the results for all the methods seem to be rather close to each other.

    The design of experiment is generally well-established. It is particularly valuable that the effects of different design choices are studied, such as using rewards and/or actions to obtain features for instance selection, considering different hyperparameters for the SELECT method etc. The results are further studied in more depth to gain insights of what instances are actually selected and why. The data and code are aimed to be made available, the experiments are described in details, which ensures replicability.
    I found it curious that the state definitions are quite different for Sigmoid and CMA-ES, particularly the last action is included in the state for Sigmoid. What is the logic behind using it for Sigmoid and not using it for CMA-ES? Is this a common approach?

    The paper is well written and nice to follow. There are just a few minor comments:
    page 6, line 582: you may want to check the alignment of "Sigmoid" and "CMA-ES" captions
    page6, line 674: an DAC --> a DAC
    page 6, line 691: it is claimed here that (MIS, Catch22, R, 0.7) configuration is the best for Sigmoid, where R stands for reward-only. However, on the line 720, page 7, it is stated that actions should be used. You may wish to check that for contradictions
    page 7, line 724: agin --> again


Scored Review Questions

	rel 	sig 	orig 	ach 	writ 	rep 	tech 	rec 	conf
pap418s2	5	4	4	5	5	5	4	5-definitely accept as full paper (5)	3

==> template/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip

